Inertial Waves in a Nonlinear Simulation of the Sun's Convection Zone and Radiative Interior

Recent observations of Rossby waves and other more exotic forms of inertial oscillations in the Sun's convection zone have kindled the hope that such waves might be used as a seismic probe of the Sun's interior. Here we present a 3D numerical simulation in spherical geometry that models the Sun's convection zone and upper radiative interior. This model features a wide variety of inertial oscillations, including both sectoral and tesseral equatorial Rossby waves, retrograde mixed inertial modes, prograde thermal Rossby waves, the recently observed high-frequency retrograde (HFR) vorticity modes, and what may be latitudinal overtones of these HFR modes. With this model, we demonstrate that sectoral and tesseral Rossby waves are ubiquitous within the radiative interior as well as within the convection zone. We suggest that there are two different Rossby-wave families in this simulation that live in different wave cavities: one in the radiative interior and one in the convection zone. Finally, we suggest that many of the retrograde inertial waves that appear in the convection zone, including the HFR modes, are in fact all related, being latitudinal overtones that are mixed modes with the prograde thermal Rossby waves.

==> Definitions.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\smallheader}[1]{\noindent\textbf{#1}}
\newcommand{\hang}{\bibitem{lab}}

% Journal Abbreviations
\newcommand{\ApJ}{ApJ}      %Astrophysical Journal
\newcommand{\apj}{ApJ}      %Astrophysical Journal
\newcommand{\ApJL}{ApJL}    %Astrophysical Journal Letters
\newcommand{\apjl}{ApJL}    %Astrophysical Journal Letters
\newcommand{\asr}{AdSpR}	%Advances in Space Research
\newcommand{\asna}{AN}		%Astronomische Nachrichten
\newcommand{\chaos}{Chaos}	%Chaos
\newcommand{\coasp}{CoASP}	%Comments on Astrophysics and Space Physics
\newcommand{\cpc}{CCoPh}	%Communications in Computational Physics
\newcommand{\fldyr}{FlDyR}	%Fluid Dynamics Research=
\newcommand{\GGG}{GGG}	 	%Geochemistry, Geophysics, Geosystems
\newcommand{\gafd}{GApFD}	%Geophysical and Astrophysical Fluid Dynamics
\newcommand{\gji}{GeoJI}	%Geophysical Journal International
\newcommand{\jats}{JAtS} 	%Journal of Atmospheric Sciences
\newcommand{\jcoph}{JCoPh}	%Journal of Computational Physics
\newcommand{\jfm}{JFM}		%Journal of Fluid Mechanics
\newcommand{\jgg}{JGG}		%Journal of Geomagnetism and Geoelectricity
\newcommand{\jpo}{JPO}		%Journal of Physical Oceanography
\newcommand{\jplph}{JPlPh}	%Journal of Plasma Physics
\newcommand{\lrsp}{LRSP}	%Living Reviews in Solar Physics
\newcommand{\natas}{NatAs}	%Nature Astronomy
\newcommand{\nucfu}{NucFu}	%Nuclear Fusion
\newcommand{\ptrslA}{RSPTA}	%Philosophical Transactions of the Royal Society of London Series A
\newcommand{\rsptA}{RSPTA}	%Philosophical Transactions of the Royal Society of London Series A
\newcommand{\phyD}{PhyD}	%Physica D
\newcommand{\phlA}{PhLA}	%Physics Letters A
\newcommand{\pepi}{PEPI}	%Physics of the Earth and Planetary Interiors
\newcommand{\phfl}{PhFl}	%Physics of Fluids
\newcommand{\plph}{PlPh}	%Plasma Physics
\newcommand{\ppcf}{PPCF}	%Plasma Physics and Controlled Fusion
\newcommand{\pnas}{PNAS}	%Proceedings of the National Academy of Science
\newcommand{\rspsa}{RSPSA}	%Proceedings of the Royal Society of London Series A
\newcommand{\qjrms}{QJRMS}	%Quarterly Journal of the Royal Meteorological Society
\newcommand{\qjmam}{QJMAM}  %Quarterly Journal of Mechanics and Applied Mathematics
\newcommand{\rasc}{RaSc}	%Radio Science
\newcommand{\rpph}{RPPh} 	%Reports on Progress in Physics
\newcommand{\sci}{Sci}		%Science
\newcommand{\scia}{SciA}	%Science Advances
\newcommand{\sgeo}{SGeo}	%Surveys in Geophysics
\newcommand{\tcfd}{ThCFD}	%Theoretical and Computational Fluid Dynamics

\newcommand{\aap}{A\&A}     %Astronomy and Astrophysics
\newcommand{\icarus}{Icarus}	%Icarus
\newcommand{\jgr}{JGR}      %Journal of Geophysics Research
\newcommand{\mnras}{MNRAS}  %Monthly Notice of the RAS
\newcommand{\nat}{Nature}   %Nature
\newcommand{\pra}{Physical Review A}
\newcommand{\pre}{Physical Review E}
\newcommand{\solphys}{Solar Physics}
\newcommand{\ssr}{Space Science Reviews}
\newcommand{\pasj}{PASJ}    %Publications of the Astronomical Society of Japan


%Colors
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\blue}[1]{{\color{blue}#1}}
\newcommand{\green}[1]{{\color{green}#1}}
\newcommand{\orange}[1]{{\color{orange}#1}}
\newcommand{\olive}[1]{{\color{olive}#1}}
\newcommand{\teal}[1]{{\color{teal}#1}}

%Derivatives and Integrals
%\newcommand{\iint}[1]{\int\limits_{~~#1}\!\!\!\!\int}
\newcommand{\der}[2][\;\;]{\ensuremath{ \frac{d{#1}}{d{#2}} }}
\newcommand{\dern}[3][\;\;]{\ensuremath{ \frac{d^{#3}{#1}}{d{#2}^{#3}} }}
\newcommand{\dpar}[2][\;\;]{\ensuremath{ \frac{\partial{#1}}{\partial{#2}} }}
\newcommand{\dparn}[3][\;\;]{\ensuremath{ \frac{\partial^{#3}{#1}}{\partial{#2}^{#3}} }}

%Vectors
\newcommand{\bvec}[1]{{\mbox{{\boldmath$#1$}}}}	% bold in mathmode
\newcommand{\unitv}[1]{\bvec{\hat{#1}}}			% bold unit vector
\newcommand{\grad}{\bvec{\nabla}}			    % bold del

%Fluid Dynamics Numbers
\newcommand{\Ek}{{\rm Ek} \,}
\newcommand{\Ra}{{\rm Ra} \,}
\newcommand{\Prandtl}{{\rm Pr} \,}
\newcommand{\Ro}{{\rm Ro} \,}

%Commonly used symbols
\newcommand{\dP}{\delta P}			% Lagrangian pressure fluctuation
\newcommand{\eps}{\varepsilon}
\newcommand{\rsun}{R_\odot}         % Solar Radius

%Equation tools
\newcommand{\D}{\displaystyle}
\newcommand{\eqnref}[1]{(\ref{#1})}

%Editing tools
\newcommand{\brad}[1]{{\color{red} #1}}
\newcommand{\nick}[1]{{\color{blue}#1}}
\newcommand{\bwh}[1]{{\color{blue} BWH: #1}}

